Interacting Tsallis agegraphic dark energy in DGP Braneworld Cosmology

The purpose of this paper is to study the Tsallis agegraphic dark energy with an interaction term between dark energy and dark matter in the DGP brane-world scenario. For this, we assume some initial conditions to obtain the dark energy density, deceleration, dark energy EoS, and total EoS parameters. Then, we analyze the statefinder parameters, $\omega'{}_{DE}-\omega_{DE}$ plots, and classical stability features of the model. The results state that the deceleration parameter provides the phase transition from decelerated to accelerated phase. The $\omega_{DE}$ graphs show the phantom behavior, while the $\omega_{tot}$ exhibits the quintessence and phantom during the evolution of the Universe. Following the graphs, the Statefinder analysis shows the quintessence behavior of the model for the past and present. However, it tends to the $\Lambda CDM$ in the following era. The $\omega'{}_{DE}-\omega_{DE}$ plot indicates the thawing or freezing area depending on the type of era and different values of $b^{2}$, $\delta$, and $m$. By the square of the sound speed, we see the model is stable in the past, stable or unstable at the current time, and unstable in the future for selected values of $b^{2}$, $\delta$, and $m$. To test the model, we use the recent Hubble data. We also employ Akaike Information Criterion (AIC) and Bayesian Information Criterion (BIC) to compare the model with the $\Lambda CDM$ as the reference model. In addition, we test the model using the $H-z$ plot, and we see a turning point in the future time. The results from the best fit values for the $\omega_{tot}$ plot emphasize that the Universe is in the quintessence region in the current time. It will enter the phantom phase, and then it will approach the $\Lambda$ state in the future. But, the $\omega_{DE}$ always stays on the phantom region. The model is unstable in the present and progressive era.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} Riess, A. G., Filippenko, A. V., Challis, P., Clocchiatti, A., Diercks, A., Garnavich, P. M., Gilliland, R. L.,  Hogan, C. J., Jha, S., \& Kirshner, R. P.: \aj \textbf{116}, 1009 (1998)

\bibitem{bib2} Perlmutter, S., Aldering, G., Goldhaber, G., Knop, R. A., Nugent, P., Castro, P. G., Deustua, S., Fabbro, S., Goobar, A., \& Groom, D. E.: \aj \textbf{517}, 565 (1999)


\bibitem{bib3} Astier, P., Guy, J., Regnault, N., Pain, R., Aubourg, E., Balam, D., Basa, S., Carlberg, R. G., Fabbro, S., Fouchez, D., Hook, I. M., Howell, D. A., Lafoux, H., Neill, J. D., Palanque-Delabrouille, N., Perrett, K., Pritchet, C. J., Rich, J., Sullivan, M., Taillet, R., Aldering, G., Antilogus, P., Arsenijevic, V., Balland, C., Baumont, S., Bronder, J., Courtois, H., Ellis, R. S., Filiol, M., Gonçalves, A. C., Goobar, A., Guide, D., Hardin, D., Lusset, V., Lidman, C., McMahon, R., Mouchet, M., Mourao, A., Perlmutter, S., Ripoche, P., Tao, C., \& Walton, N.: \aap \textbf{447}, 31-48 (2006)

\bibitem{bib4} Riess, A. G., Kirshner, R. P., Schmidt, B. P., Jha, S., Challis, P., Garnavich, P. M., Esin, A. A., Carpenter, C., Grashius, R., \& Schild, R. E.: \apj \textbf{117}, 707 (1999)

\bibitem{bib5} Amanullah, R., Lidman, C., Rubin, D., Aldering, G., Astier, P., Barbary, K., Burns, M. S., Conley, A., Dawson, K. S., \& Deustua, S. E.: \apj \textbf{716}, 712 (2010)


\bibitem{bib6} Randall, L., \& Sundrum, R.: \prl \textbf{83}, 3370 (1999)


\bibitem{bib7} Randall, L., \& Sundrum, R.: \prl \textbf{83}, 4690 (1999)

\bibitem{bib8} Dvali, G. R., Gabadadze, G., \& Porrati, M.: Phys. Lett.
B \textbf{485}, 208 (2000)


\bibitem{bib9} Sahni, V., \& Starobinsky, A.A.: Int. J. Mod. Phys. D 9, 373 (2000)

\bibitem{bib10} Peebles, P.J.E., \& Ratra, B.:  Rev. Mod. Phys. \textbf{75}, 559 (2003)


\bibitem{bib11} Copeland, E. J., Sami, M., \& Tsujikawa, S.: Int. J. Mod. Phys., D \textbf{15}, 1753 (2006)


\bibitem{bib12} Armendariz-Picon, C., Mukhanov, V.F., \& Steinhardt, P.J.: \prl \text{85}, 4438 (2000)

\bibitem{bib13} Kamenshchik, A.Y., Moschella, U., \& Pasquier, V.: Phys. Lett. B \text{511}, 265 (2001)

\bibitem{bib14} Caldwell, R.R.: Phys. Lett. B \textbf{545}, 23 (2002)



\bibitem{bib15} Cai, R. G.: Phys. Lett. B \textbf{657}, 228 (2007)

\bibitem{bib16} Wei, H. \& Cai, R. G.: Phys. Lett. B \textbf{660}, 113 (2008)

\bibitem{bib17} Wei, H.\& Cai, R.-G.: Phys. Lett. B\textbf{663}, (2008). arXiv:0708.1894

\bibitem{bib18} Liu, X.-L., Zhang, X.: Commun. Theor. Phys. \textbf{52} (2009). arXiv:0909.4911

\bibitem{bib19} Jamil, M., Saridakis, E. N.: JCAP \textbf{1007}, 028 (2010). arXiv:1003.5637

\bibitem{bib20} Saaidi, K., Sheikhahmadi, H., \& Mohammadi, A. H.: \apss \textbf{338} (2012). arXiv:1201.0275

\bibitem{bib21} Tsallis, C., Cirto, L. J.L.: Eur. Phys. J. C \textbf{73}, 2487 (2013). arXiv:1202.2154

\bibitem{bib22} Barrow, J. D.: Phy. Lett. B\textbf{808}, 135643 (2020). https://doi
    .org/10.1016/j.physletb.2020.135643

\bibitem{bib23} Moradpour, H., Corda, C., Ziaie, A. H. \& Ghaffari, S.: EPL \textbf{127}, 60006 (2019)


\bibitem{bib24} Shababi, H. \& Ourabah, K.: Eur. Phys. J. Plus \textbf{135}, 697 (2020). https://doi.org/10.1140/epjp/s13360-020-00726-9

\bibitem{bib25} Abdollahi Zadeh, M., Sheykhi, A., \& Moradpour, H.: Modern Physics Letters A \textbf{34}, 1950086 (2019).\\ arXiv:1810.12104

\bibitem{bib26} Srivastava, Sh., Dubey, V. C., \& Sharma, U. K.: Int. J. Mod. Phys. A \textbf{35}, 2050027 (2020)

\bibitem{bib27} Xu, Y D.: Commun. Theor. Phys. \textbf{72}, 015402 (2020). https://doi.org/10.1088/1572-9494/ab544e

\bibitem{bib28} Dvali, G., Gabadadze, G., \& Porrati, M.: Phys. Lett. B \textbf{485}, 208 (2000). arXiv:hep-th/0005016


\bibitem{bib29} Deffayet, C.: Phys. Lett. B \textbf{502}, (2001). arXiv:hep-th/0010186

\bibitem{bib30} Deffayet, C., Dvali, G.R., \& Gabadadze,G.: \prd \textbf{65}, 044023 (2002). arXiv:astro-ph/0105068


\bibitem{bib31} Hu, B. \& Ling, Y.: \prd \textbf{73}, 123510 (2006)

\bibitem{bib32} Chimento, L.P. \& Richarte, M.G.: \prd \textbf{85}, 127301 (2012)

\bibitem{bib33} Ebrahimi, E., Golchin, H., Mehrabi, A., \& Movahed, S.M.S.: Int. J. Mod. Phys. D \textbf{26},1750124 (2017). https://doi.org/
    10.1142/S0218271817501243

\bibitem{bib34} Arévalo, F., Bacalhau, A. P. R., \& Zimdahl, W.: Class. Quantum Grav. \textbf{29}, 235001 (2012). arXiv:1112.5095



\bibitem{bib35} Sheykhi, A., Dehghani, M. H., \& Ghaffari, S.: Int. J. Mod. Phys. D, \textbf{25}, 1650018 (2016). arXiv:1506.02505

\bibitem{bib36} Maartens, R. \& Koyama, K.: Living Rev. Relativ. \textbf{13}, 5 (2010). https://doi.org/10.12942/lrr-2010-5



\bibitem{bib37} Amarilla, L. \& Eiroa, E. F.: \prd \textbf{85}, 064019 (2012)



\bibitem{bib38} Sheykhi, A. \& Wang, B.: Mod. Phys. Lett. A \textbf{25}, 1199 (2010)


\bibitem{bib39} Sheykhi, A., Dehghani, M. H., \& Hosseini, S. E.: Phys. Lett. B \textbf{726}, 23 (2013)



\bibitem{bib40} Planck Collaboration: A\&A \textbf{641}, (2020).  https://doi.org/10.1051/0004-6361/201833910


\bibitem{bib41} Rani, S.; Azhar, N.: Universe \textbf{7}, 268 (2021). https://doi.org/10.3390/universe7080268

\bibitem{bib42} Moresco, M., Pozzetti, L., Cimatti, A., Jimenez, R., Maraston, C., Verde, L., Thomas, D., Citro, A., Tojeiro, R., \& Wilkinson, D.: JCAP \textbf{05}, 014 (2016). arXiv:1601.01701

\bibitem{bib43} Sadri, E. \& Khurshudyan, M.: Int. J. Mod. Phys. D\textbf{28}, 1950152 (2019). arXiv:1809.07595


\bibitem{bib44} Ghaffari, S., Moradpour, H., Bezerra, V. B., Morais Gra\c{c}a, J.P., \& Lobo, I.P.: Phys. Dark Universe \textbf{23}, 100246 (2019)

\bibitem{bib45} Ghaffari, S., Dehghani, M. H., \& Sheykhi, A.: \prd \textbf{89}, 123009 (2014)

\bibitem{bib46} Gumjudpai, B.: Gen Relativ Gravit\textbf{36}, 747–766 (2004).  https://doi.org/10.1023/B:GERG.0000016922.72972.67

\bibitem{bib47} Jawad, A., Rani, S., Salako, I. G., \& Gulshan, F.: Eur. Phys. J. Plus \textbf{131}, 236 (2016). https://doi.org/10.1140/epjp/
    i2016-16236-x

\bibitem{bib48} Salvatelli, V., Said, N., Bruni, M., Melchiorri, A., \& Wands, D.: \prl \textbf{113}, 181301 (2014). arXiv:1406.7297

\bibitem{bib49} Holden, D. J. \& Wands, D.: \prd\textbf{61}, 043506 (2000). arXiv:gr-qc/9908026

\bibitem{bib50} Farrar, G. R. \& Peebles, P. J. E.: \apj \textbf{604}, 1 (2004). arXiv:astro-ph/0307316

\bibitem{bib51} Copeland, E. J., Liddle, A. R. \& Wands, D.: \prd \textbf{57}, 4686 (1998). arXiv:gr-qc/9711068

\bibitem{bib52} Uzan, J.-P.: \prd \textbf{59}, 123510 (1999). arXiv:gr-qc/9903004

\bibitem{bib53} Amendola, L.: \prd \textbf{62}, 043511 (2000). astro-ph/9908023

\bibitem{bib54} Bean, R. \& Magueijo, J.: Phys. Lett. B\textbf{517}, 177 (2001). arXiv:astro-ph/0007199

\bibitem{bib55} Bean, R.: \prd \textbf{64}, 123516 (2001)

\bibitem{bib56} Das, S., Corasaniti, P. S. \& Khoury, J.: \prd \textbf{73},
083509 (2006). astro-ph/0510628

\bibitem{bib57} Lee, S., Liu, G.-C. \& Ng, K.-W.: \prd \textbf{73},
083516 (2006). astro-ph/0601333

\bibitem{bib58} Copeland, E. J., Sami, M. \& Tsujikawa, S.: Int. J. Mod. Phys. D\textbf{15}, 1753 (2006). arXiv:hep-th/0603057



\bibitem{bib59} Akama, A.: Lect. Notes Phys.\textbf{176}, 0001113 (1982)



\bibitem{bib60} Pavon, D. \& Zimdahl, W.: Phys. Lett. B \textbf{628}, (2005)

\bibitem{bib61} Sadeghi, J., Khurshudyan, M., Movsisyan, A., \& Farahani, H.: JCAP \textbf{12}, 031 (2013)

\bibitem{bib62} Honarvaryan, M., Sheykhi, A., \& Moradpour, H.: Int. J. Mod. Phys. D \textbf{24}, 1550048 (2015). https://doi.org/10.1142/S0218271815500480

\bibitem{bib63} Abdollahi Zadeh, M., Sheykhi, A., Moradpour, H., \& Bamba, K.: Eur. Phys. J. C \textbf{78}, 940 (2018). \\https://doi.org/10.1140/epjc/s10052-018-6427-3

\bibitem{bib64} Sadri, E.: Eur. Phys. J. C \textbf{79}, 762 (2019).  https://doi.org/10.1140/epjc/s10052-019-7263-9


\bibitem{bib65} Wang, B., Zang, J., Lin, C.-Y., Abdalla, E., \& Micheletti, S.: Nuclear Physics B \textbf{778}, (2007)


\bibitem{bib66} Sheykhi, A., Sadegh Movahed, M., \& Ebrahimi, E.: \apss \textbf{339}, 93–99(2012) . https://doi.org/10.1007/s10509-012-0977-x

\bibitem{bib67} Srivastava, S., Sharma, U., \& Dubey, V.: Gen Relativ Gravit \textbf{53}, 47 (2021). https://doi.org/10.1007/s10714-021-02818-y




\bibitem{bib68} Sahni, V., Saini, T.D., Starobinsky, A.A., \& Alam, U.: Jetp Lett. \textbf{77}, 201–206 (2003). https://doi.org/
    10.1134/1.1574831


\bibitem{bib69} Caldwell, R.R. \& Linder, E.V.: \prl \textbf{95}, 141301 (2005)


\bibitem{bib70} Akaike, H.: IEEE Transactions on Automatic Control \textbf{19}, 716-723 (1974). doi: 10.1109/TAC.1974.1100705
    
\bibitem{bib71} Schwarz, G.: Annals of Statistics \textbf{6}, 461-464 (1978).  http://dx.doi.org/10.1214/aos/1176344136


\bibitem{bib72} Colga\'in, E. O\', Sheikh-Jabbari,  M. M.: Class. Quantum Grav. \textbf{38}, 177001 (2021)


\bibitem{bib73} Huang, Q., Huang, H., Xu, B., Tu, F., Chen, J.: Eur. Phys. J. C \textbf{81}, 686 (2021). https://doi.org/10.1140/epjc/s10052\\-021-09480-3


\bibitem{bib74} Anagnostopoulos, F. K., Basilakos, S., Saridakis, E. N.: Eur. Phys. J. C \textbf{80}, 826 (2020)

 
    
    

\end{thebibliography} 
